Deadline Scheduling as Restless Bandits

The problem of stochastic deadline scheduling is considered. A constrained Markov decision process model is introduced in which jobs arrive randomly at a service center with stochastic job sizes, rewards, and completion deadlines. The service provider faces random processing costs, convex non-completion penalties, and a capacity constraint that limits the simultaneous processing of jobs. Formulated as a restless multi-armed bandit problem, the stochastic deadline scheduling problem is shown to be indexable. A closed-form expression of the Whittle's index is obtained for the case when the processing costs are constant. An upper bound on the gap-to-optimality for the Whittle's index policy is obtained, and it is shown that the bound converges to zero as the job arrival rate and the number of available processors increase simultaneously to infinity.

==> finitePerformance.tex <==
In this section, we examine the performance of Whittle's index policy for the stochastic deadline scheduling problem when the number of servers ($M$) is finite.  We show that when${M<N}$, there does not exist an optimal index policy, hence Whittle's index policy is not optimal.   We further derive an upper bound on the gap-to-optimality on the performance of the Whittle's index policy.  This result provides the essential ingredient for establishing asymptotic optimality of Whittle's index policy in Section \ref{sec:V}.

%
%
%(I suggest we deemphasize Theorem 3 and LLLP extension.)
%
%
%
%In this section, we examine the performance of the Whittle's index policy for the stochastic deadline scheduling problem.
% In Theorem ~\ref{thm:optimal}, we establish the optimality of
% the Whittle's index policy for an important special case with ${M=N}$.
%  When ${M<N}$, a counter-example is given to show that
%  there does not exist an optimal index policy in general.
% %In Section \ref{sec:op3}, we establish the asymptotic optimality of
%%  the Whittle's index policy in the light traffic regime.
%In Section \ref{sec:op4}, we apply the
%Least Laxity and Longer Processing Time (LLLP) principle (originally proposed in \cite{Xu&Pan:2012CDC}) to
%improve the the Whittle's index policy.


\subsection{Performance in the Finite Processor Cases}\label{sec:op1}
In general, Whittle's index policy is not optimal except in some special cases \cite{Liu&Zhao:08ITsub}.  For the deadline scheduling problem, the same conclusion holds. We show in fact that no index policy exists.



\begin{thm}\label{thm:optimal}
When ${M=N}$, the Whittle's index policy is optimal for the RMAB problem formulated in (\ref{eqn:MAB}).
When ${M<N}$, an optimal index policy does not exist in general.
\end{thm}
For the ${M=N}$ case, the formal proof of the optimality can be found in Appendix \ref{proof:optimalityOfWhittleIndexPolicy}.
For the ${M<N}$ case, we show, by counter examples, that index policy does not exist in general unless additional constraints are imposed to the model.

An {\it index policy} assigns each job an index (that depends only on the job's current state),
and processes the jobs with the highest indices \cite{Gittins:79JRSS}.
The Whittle's index policy is an example of index policies, and thus is sub-optimal.


Set the capacity of the queue to be ${N=3}$, the number of processors ${M=1}$, the discounted factor ${\beta=0.4}$, the penalty function ${F(B)=B^2}$, and the processing cost ${c[t]=1}$. Assume the arrival is busy $(Q(0,0)=0)$ and the initial laxity is zero ($T=B$ at arrival). For this small scale MDP, a linear programming formulation is used to solve for the optimal policy \cite{Ross:book2014}.


 Consider two different states,
 \[
 \begin{array}{ll}
 {s=((1,1),(2,2),(2,2))}\\
 {s'=((1,1),(1,1),(2,2))}
 \end{array}
 \]
where ${s=((T_1,B_1),(T_2,B_2),(T_3,B_3))\in\mathcal{S}}$ is the state of the system including the states of each arm.

 For state $s$, the optimal action is to process job $(2,2)$. The job $(2,2)$ is preferred to $(1,1)$ in this case. Processing $(2,2)$ will cause $1$ instant penalty, and the state will change to ${((T,B),(1,1),(1,2))}$, where $(T,B)$ is a new arrival. In next stage, a penalty of $2$ from the last two jobs will happen. If some policy processes $(1,1)$ alternately, there will be no penalty in the first stage and the state will change to ${((T,B),(1,2),(1,2))}$. The last two jobs will at lease incur a penalty of $5$.

 For state $s'$, the optimal action is to process the job $(1,1)$. The job $(1,1)$ is preferred to $(2,2)$ in this case. Processing $(1,1)$ will cause $1$ instant penalty, and the state will change to ${((T,B),(T',B'),(1,2))}$, where $(T,B)$ and $(T',B')$ are new arrivals. If some policy processes $(2,2)$ alternately, there will an instant penalty of $2$ from the first two jobs in the first stage and the state will change to ${((T,B),(T',B'),(1,1))}$. In this case, a penalty of $1$ can be saved by processing $(2,2)$ in the previous stage. However, due to the discount factor, it is more profitable to process $(1,1)$.

 For any ``index'' policy, the indices of job $(1,1)$ and $(2,2)$ are fixed and the preference of these two jobs should remain the same in these two cases, which is violated by the result here. This counter example shows that no ``index'' policy that is optimal in general.



\subsection{An Upper Bound of the Gap-to-Optimality}\label{sec:op3}
%Although the Whittle's index policy is not optimal in general, it is shown to be asymptotically optimal when both the job traffic and the processing capacity scale while the system stays stable.
In the following theorem, we first establish a result that applies quite generally to the case for a  finite queue size $N$ and finite $M$ number of processors.



\begin{thm}\label{thm:gap}
Let $G^N(s)$ be the optimal value function defined in (\ref{eqn:originPro}) and $G^N_{\scriptsize\mbox{RMAB}}(s)$ be the value function achieved by the Whittle's index policy, respectively.  We have
  \beq\label{eqn:bound}
  %G(s)-G_{\pi_M}(s)\le \frac{C}{1-\beta}\mathbb{E}[I[t]\mathbbm{1}(I[t]>M)]
  G^N(s)-G^N_{\scriptsize\mbox{RMAB}}(s)\le \frac{C}{1-\beta}\mathbb{E}[I^N[t]\mathds{1}(I^N[t]>M)],
  \eeq
  where $I^N[t]$ is the number of jobs admitted in the queue with $N$ positions within time $[t-\bar{T}+1,t]$, $\bar{T}$ is the maximum lead time of jobs, and $C$ is a constant determined by the processing cost and the penalty of non-completion.
  \end{thm}


The proof can be found in Appendix \ref{proof:asymptotic}. The gap-to-optimality is bounded by the tail expectation of the jobs admitted to the system. Note that, the conditional expectation on the right hand side (RHS) of (\ref{eqn:bound}) is connected to the conditional value at risk (CVaR) \cite{Rockafellar&Uryasev:2000JR}, which measures the expected losses at a certain risk level and is extremely important in the risk management.




\subsection{Least Laxity and Longer Processing Time (LLLP) Principle}\label{sec:op4}
\input scheduling_v4.tex


